An Empirical Study on Bug Severity Estimation using Source Code Metrics and Static Analysis

In the past couple of decades, significant research efforts have been devoted to the prediction of software bugs (i.e., defects). In general, these works leverage a diverse set of metrics, tools, and techniques to predict which classes, methods, lines, or commits are buggy. However, most existing work in this domain treats all bugs the same, which is not the case in practice. The more severe the bugs the higher their consequences. Therefore, it is important for a defect prediction method to estimate the severity of the identified bugs, so that the higher severity ones get immediate attention. In this paper, we provide a quantitative and qualitative study on two popular datasets (Defects4J and Bugs.jar), using 10 common source code metrics, and two popular static analysis tools (SpotBugs and Infer) for analyzing their capability to predict defects and their severity. We studied 3,358 buggy methods with different severity labels from 19 Java open-source projects. Results show that although code metrics are useful in predicting buggy code (Lines of the Code, Maintainable Index, FanOut, and Effort metrics are the best), they cannot estimate the severity level of the bugs. In addition, we observed that static analysis tools have weak performance in both predicting bugs (F1 score range of 3.1%-7.1%) and their severity label (F1 score under 2%). We also manually studied the characteristics of the severe bugs to identify possible reasons behind the weak performance of code metrics and static analysis tools in estimating their severity. Also, our categorization shows that Security bugs have high severity in most cases while Edge/Boundary faults have low severity. Finally, we discuss the practical implications of the results and propose new directions for future research.

==> abstract.tex <==
\begin{abstract}
In the past couple of decades, significant research efforts have been devoted to the prediction of software bugs (i.e., defects). In general, these works leverage a diverse set of metrics, tools, and techniques to predict which classes, methods, lines, or commits are buggy. However, most existing work in this domain treats all bugs the same, which is not the case in practice. The more severe the bugs the higher their consequences. Therefore, it is important for a defect prediction method to estimate the severity of the identified bugs, so that the higher severity ones get immediate attention. 
In this paper, we provide a quantitative and qualitative study on two popular datasets (Defects4J and Bugs.jar), using 10 common source code metrics, and two popular static analysis tools (SpotBugs and Infer) for analyzing their capability to predict defects and their severity. We studied 3,358 buggy methods with different severity labels from 19 Java open-source projects. Results show that although code metrics are useful in predicting buggy code (Lines of the Code, Maintainable Index, FanOut, and Effort metrics are the best), they cannot estimate the severity level of the bugs. In addition, we observed that static analysis tools have weak performance in both predicting bugs (F1 score range of 3.1\%-7.1\%) and their severity label (F1 score under 2\%). 
We also manually studied the characteristics of the severe bugs to identify possible reasons behind the weak performance of code metrics and static analysis tools in estimating their severity. Also, our categorization shows that Security bugs have high severity in most cases while Edge/Boundary faults have low severity. Finally, we discuss the practical implications of the results and propose new directions for future research. 
\end{abstract}

==> background.tex <==
\subsection{Source Code Metrics}
\textcolor{blue}{Intuitively, if a code component does most of the work, is more complex, and contains source code-induced code smells, that code component is likely to contain bugs. Consequently, different source code metrics with module-level, class-level, and method-level granularities have been used to measure software quality and predict bugs in previous research~\cite{giger2012method,pecorelli2019comparing,pascarella2020performance, gil2017correlation, chowdhury-method-2024, chowdhury2022revisiting}. These metrics generally focus on how large, complex, readable, and testable a code component is. The success of these code metrics in estimating maintenance efforts, such as predicting bugs, has been historically debated~\cite{chowdhury2022revisiting}. In recent research, however, it was discovered that although code metrics are not useful in understanding software maintenance at the class/file level~\cite{gil2017correlation}, they are very helpful in understanding maintenance in the method-level source code granularity~\cite{landman2014empirical, chowdhury2022revisiting}. Then again, this observation contradicts another recent study by Pascarella~\cite{pascarella2020performance} al., who observed negative results while building code metrics-based method-level bug prediction models. None of these previous studies, however, investigate if code metrics are useful to understand bug severity. \emph{Perhaps, a bug inside a more complex method is more severe than a bug contained in a simpler method.} In this paper, we, therefore, not only investigate code metrics' effectiveness in detecting/predicting bugs at the method level but also their usefulness in understanding bug severity.}   

We leverage most of the common method-level source code metrics that are used in the previous research (mentioned in the \hyperref[sec:Related Work]{Related Work} section) to see their capability in predicting buggy codes and their severity. Although the list of selected metrics is not exhaustive (given the numerous metrics explored in this field and the limitations of experiment size in one article), but we made sure we have most of the metrics that have been shown effective in predicting the method-level bugginess, in the past.  These metrics are defined as follows:

\textbf{Lines of Code (LC)}: Size, also known as lines of code (LC), is the most popular, easy to measure, and the most effective code metric for estimating software maintenance~\cite{Gil:2017,Emam:2001,chowdhury:2022}.  
The use of LC as a proxy maintenance indicator is so prevalent that there are dedicated studies that completely focus on LC and its correlation with other quality metrics (e.g., ~\cite{Gil:2017,landman2014empirical,chowdhury:2022}). LC has been extensively studied for bug prediction, fault localization, and for finding vulnerabilities (e.g.,~\cite{chowdhury-method-2024,pascarella2020performance,antinyan2014identifying,shin2010evaluating,chowdhury:2022}). In this paper, we calculate LC as the source lines of code without comments and blank lines, similar to~\cite{landman2014empirical,ralph2018construct,chowdhury:2022} to prevent the code formatting and comments effects, which are out of this study scope.

\textbf{McCabe (MA)}: McCabe \cite{mccabe1976complexity,landman2014empirical}, also known as cyclomatic complexity, is another very popular metric that indicates the number of independent paths, and thus the logical complexity of a program. Intuitively, components with high McCabe values are more bug-prone. McCabe has been studied extensively to find bugs and locate suspicious code~\cite{antinyan2014identifying}, to understand its correlation with code quality~\cite{pantiuchina2018improving}, and to leverage its value for test generation methods, such as structured testing (path testing)~\cite{watson1996structured}. McCabe can be calculated as $1 + \#predicates$~\cite{mccabe1976complexity}.

\textbf{McClure (ML)}: McClure \cite{mcclure1978model,kafura1987use} was proposed as an improvement over McCabe. Unlike McCabe, McClure considers the number of control variables, and the number of comparisons in a predicate, which is not supported by McCabe. Intuitively, a predicate with multiple comparisons and multiple control variables would be more complex, and thus more bug-prone, than a predicate with only one comparison or only a single control variable. 


\textbf{Nested Block Depth (NBD)}: McCabe and McClure do not consider nested depth. According to these metrics, there is no difference between two code snippets containing two identical for loops if they are arranged serially or nested. NBD~\cite{kasto2013measuring,alenezi2019impact,zaw2020software} has been studied alongside McCabe and McClure to alleviate this issue. 

\textbf{Proxy Indentation (PI)}: Since McCabe-like complexity measures require a language-specific parser (for finding the predicates), Hindle et al. \cite{hindle2008reading} proposed Proxy Indentation metric as a proxy for McCabe-like complexity metrics. It was shown that, for measuring 
complexity, indentation measurement can perform very similar to more complex measurements such as McCabe, without requiring a language-specific
parser. Indentation measurement is done for each line, and then an aggregated value is calculated for the whole program component (e.g., a method).
Hindle et al. showed that the standard deviation as an aggregated value outperforms mean, median or max.

\textbf{FanOut (FO)}: This metric calculates the total number of methods called a given method. This provides an estimate of the coupling---i.e., dependency of a particular method on other methods. It is observed that code components that are highly coupled are less maintainable and bug-prone~\cite{mo2016decoupling,alomar2019impact}.

\textbf{Readability (R)}: This metric combines different code features to calculate a single value for estimating code readability. We used the readability metric proposed by Buse et al.~\cite{buse2009learning} which generates a readability score for a given method. The readability scores range from 0 to 1 for specifying least readable code to most readable code, respectively. The authors concluded that this metric has a significant level of correlation with defects, code churn, and self-reported stability.

\textbf{Halstead Metrics}: The Halstead code metrics contain seven measures based on the number of operators and operands in a component \cite{halstead1977elements}. These metrics have been used in different research such as measuring code complexity perceived by developers~\cite{antinyan2017evaluating}, calculating the complexity of software maintenance tasks~\cite{curtis1979measuring,kafura1987use}, finding their correlation with indentation measures~\cite{hindle2008reading}, and estimating software readability ~\cite{posnett2011simpler}. As all the Halstead metrics are highly correlated to each other, so in this paper, we consider only two of them: \textbf{Difficulty (D)} and \textbf{Effort (E)} which use other Halstead metrics in their formulas.
The Halstead Difficulty is calculated as shown in Eq\ref{Eq1}


%\begin{displaymath}
\begin{equation} \label{Eq1}
D = \frac{n1}{2} * \frac{N2}{n2}
\end{equation}
%\end{displaymath}


Where ~$n1$ is the number of distinct operators, ~$n2$ is the number of distinct operands, and ~$N2$ is the total number of operands.\\

The Halstead Effort is calculated as shown in Eq\ref{Eq1}and \ref{Eq2}
%\begin{fleqn}
\begin{equation}\label{Eq2}
\begin{split}
%\begin{aligned}
&E = D * V\\
&V = N * \log_2 (n)\\
&N = N1 + N2\\
&n = n1 + n2
\end{split}
%\end{aligned}
\end{equation}
%\end{fleqn}

Where ~$N1$ is the total number of operators.\\

\textbf{Maintainability Index (MI)}: 
The Maintainability Index has been introduced by Omran and Hagemeister~\cite{oman1992metrics} where the authors defined metrics for measuring 
the maintainability of a software system and combine those metrics into a single value. This metric has evolved over time and was adopted by popular tools like Visual Studio~\cite{visual_studio}. 
MI calculated as shown in Eq\ref{Eq3}. 

\begin{equation}\label{Eq3}
\begin{split} 
%\begin{multline*}
&MI= 171- 5.2 ∗  ln(HalsteadVolume)- \\
&0.23 ∗ (McCabe)− 16.2 * ln(LOC)
\end{split}
%\end{multline*}
\end{equation}
\\
Table \ref{tab:metrics_overview} provides a brief description for each of our 10 studied metrics with their abbreviation.

\begin{table*}[tbp]
    \caption{
\label{tab:metrics_overview} List of studied metrics and their brief description.}
    \begin{center}
      \begin{tabular}{p{1cm} p{12cm}}
        \toprule
        \textbf{Metric} & \textbf{Description}\\
        \midrule
        LC & Number of source code lines without comments and blank lines \\
        MA & Number of independent paths (logical complexity) \\
        ML & Number of control variables and number of comparisons in a predicate\\
        NBD & Counting the depth of most nested block\\
        PI & Counting indentation of source code lines\\
        FO & Counting total number of methods called a given method\\
        R& Measuring the readability of the code in the range of 0-1 (least to most)\\
        D & Measure the difficulty of the program to write or understand the code\\
        E & Determining the required effort for developing/maintaining the code\\
        MI & Measuring how much the code is maintainable\\
        
        \bottomrule
      \end{tabular}
    \end{center}
  \end{table*}
  
  
\subsection{Static Analysis Tools}
Static analysis tools have been introduced for finding bugs by using different techniques, such as pattern matching. \textbf{FindBugs}~\cite{findbugs} is an open-source tool that analyzes Java byte code for finding bugs. \textbf{SpotBugs}~\cite{spotbugs} is a successor of FindBugs which is actively under maintenance. SpotBugs has more than 400 bug patterns and their description is available on the tool's website \cite{spotbugs}. \textbf{Infer} \cite{infer} is a static analysis tool for different programming languages such as Java, C++, Objective-C, and C, which is also actively maintained. Infer has more than 100 predefined issue types which are described on its website \cite{infer}.
\textbf{Error prone}~\cite{error_prone} is another static analysis tool from Google which is used for Java code to catch common programming faults at the compile-time, and it is actively under maintenance. We have selected SpotBugs and Infer tools for our study because of their extensive usage in the previous studies and in practice, and we exclude the ErrorProne because its latest versions do not support older versions of Java projects which exist in our datasets. A more detailed explanation of our selected configuration for these tools is explained in Section~\ref{static-tools}.

